Validating Static Warnings via Testing Code Fragments

Static analysis is an important approach for finding bugs and vulnerabilities in software. However, inspecting and confirming static warnings are challenging and time-consuming. In this paper, we present a novel solution that automatically generates test cases based on static warnings to validate true and false positives. We designed a syntactic patching algorithm that can generate syntactically valid, semantic preserving executable code fragments from static warnings. We developed a build and testing system to automatically test code fragments using fuzzers, KLEE and Valgrind. We evaluated our techniques using 12 real-world C projects and 1955 warnings from two commercial static analysis tools. We successfully built 68.5% code fragments and generated 1003 test cases. Through automatic testing, we identified 48 true positives and 27 false positives, and 205 likely false positives. We matched 4 CVE and real-world bugs using Helium, and they are only triggered by our tool but not other baseline tools. We found that testing code fragments is scalable and useful; it can trigger bugs that testing entire programs or testing procedures failed to trigger.

==> tikz-grammar.tex <==
\setlength{\grammarparsep}{1pt plus 1pt minus 1pt}
\setlength{\grammarindent}{11em}


\begin{figure*}[ht!]
  \centering
  \begin{tikzpicture}[every node/.style={
      text width=15cm,anchor=north west,
      node distance=-5pt
    }]
    \node(bnf1) {
      \begin{grammar}
        <translation-unit> ::= <external-declaration>
        | <translation-unit> <external-declaration>
        <external-declaration> ::= <function-definition> | <declaration>
        <function-definition> ::=
        <declaration-specifiers> <declarator> <declaration-list>$_{opt}$ <compound-statement>
      \end{grammar}
    };
    \node(bnf2)[below=of bnf1] {
      \begin{grammar}
        <statement> ::=
        <labeled-statement>
        | <compound-statement>
        | <expression-statement>
        \alt <selection-statement>
        | <iteration-statement>
        | <jump-statement>
      \end{grammar}
    };

    \node(bnf3)[below=of bnf2] {
      \begin{grammar}
        <compound-statement> ::= `{' <block-item-list>$_{opt}$ `}'
        <block-item-list> ::= <block-item> | <block-item-list> <block-item>

        <block-item> ::= <declaration> | <statement>

        <declaration> ::= <declaration-specifiers> <init-declarator-list>$_{opt}$ `;'

        <init-declarator-list> ::= <init-declarator> | <init-declarator-list> `,' <init-declarator>

        <init-declarator> ::= <declarator> | <declarator> `=' <initializer>

      \end{grammar}
    };

    \node (bnf4) [below=of bnf3] {
      \begin{grammar}
        <expression-statement> ::= <expression>$_{opt}$ `;'

        <expression> ::= <assignment-expression>
        | <expression> `,' <assignment-expression>

        <assignment-expression> ::= <conditional-expression>
        \alt <unary-expression> <assignment-operator> <assignment-expression>

        <conditional-expression> ::= ... ::= <additive-expression> ::= ... ::= <primary-expression>

        <additive-expression> ::= <multiplicative-expression>
        \alt <additive-expression> `+' <multiplicative-expression>
        \alt <additive-expression> `-' <multiplicative-expression>

        <unary-expression> ::= ... ::= <primary-expression>

        <primary-expression> ::= <identifier> | <constant> | <string-literal> | `(' <expression> `)'

        <assignment-operator> ::=
        `=' | `*=' | `/=' | `\%=' ...
      \end{grammar}
    };
    \node (bnf5) [below=of bnf4] {
      \begin{grammar}
        <labeled-statement> ::=
        <identifier> `:' <statement>
        \alt `case' <constant-expression> `:' <statement>
        \alt `default' `:' <statement>

        <selection-statement> ::=
        `if' `(' <expression> `)' <statement>
        \alt `if' `(' <expression> `)' <statement> `else' <statement>
        \alt `switch' `(' <expression> `)' <statement>

        <iteration-statement> ::=
        `while' `(' <expression> `)' <statement>
        \alt `do' <statement> `while' `(' <expression> `)' `;'
        \alt `for' `(' <expression>$_{opt}$ `;' <expression>$_{opt}$ `;' <expression>$_{opt}$ `)' <statement>
        \alt `for' `(' <declaration> <expression>$_{opt}$  `;' <expression>$_{opt}$ `)' <statement>

        <jump-statement> ::=
        `goto' <identifier> `;'
        | `continue' `;'
        | `break' `;'
        \alt `return' <expression>$_{opt}$ `;'

      \end{grammar}
    };
    \draw (bnf1.south west) -- (bnf1.south east);
    \draw (bnf2.south west) -- (bnf2.south east);
    \draw (bnf3.south west) -- (bnf3.south east);
    \draw (bnf4.south west) -- (bnf4.south east);

  \end{tikzpicture}
  \caption{Part of C99 Grammar\label{fig:grammar-c99}}
\end{figure*}

